Enhancing LLMs in Predictive Political QA with Semi-Structured Data

Predictive political question answering (QA), such as predicting how a political actor will vote, goes beyond factual lookup. External political resources offer rich historical evidence, but rarely contain the answer itself. Existing LLM augmentation methods, including actor-profile-based simulation and knowledge graph evidence injection, improve political reasoning but largely treat external resources as knowledge-based evidence, leaving prediction-relevant signals under-modeled. We identify two complementary signals for predictive political QA: actor stances that capture issue-specific preferences, and high-order structure signals that capture indirect dependencies among political actors. We propose PSL, a dual-view framework that converts semi-structured political records into inference-oriented evidence for LLMs. PSL extracts stance signals from question-relevant actor records in a semantic view, and learns structure-aware actor representations from an actor interaction graph in a vector view. Across three real-world datasets and multiple LLMs, PSL consistently outperforms baselines, with ablations confirming the complementary gains of stance and structure signals.

==> fig_table/combined_neighbor_context_and_retrieval.tex <==
\begin{figure*}[!t]
  \centering
  % === 左侧：图片部分 (占约 66% 宽度) ===
  \begin{minipage}[b]{0.58\textwidth}
    \centering
    % 图例
    \begin{subfigure}[b]{\linewidth}
      \centering
      % 建议图例宽度稍微改小一点，避免边缘溢出
      \includegraphics[width=0.9\linewidth]{fig_table/neighbor_context_legend.pdf}
    \end{subfigure}
    \vspace{-1.3em}

    % 三张子图
    \begin{subfigure}[b]{0.32\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig_table/neighbor_context_rcvp.pdf}
      \caption{RCVP}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.32\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig_table/neighbor_context_icews.pdf}
      \caption{ICEWS}
    \end{subfigure}\hfill
    \begin{subfigure}[b]{0.32\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig_table/neighbor_context_staid.pdf}
      \caption{StaId}
    \end{subfigure}
    
    \vspace{-0.5em}
    \caption{Performance of PSL using different numbers of political actors’ neighbors and their records in the form of text.}
    \label{p2}
  \end{minipage}%
  \hfill % 左右两栏之间的弹性间距
  % === 右侧：表格部分 (占约 32% 宽度) ===
  \begin{minipage}[b]{0.36\textwidth}
    \centering
    % 【重要】将 caption 类型强制改为 table
    \makeatletter\def\@captype{table}\makeatother 
    
    % 使用 resizebox 让表格自动适应窄宽度
    \resizebox{\linewidth}{!}{
      \begin{tabular}{lrrr}
      \toprule
      \textit{\textbf{Variant}} & \textit{\textbf{RCVP}} & \textit{\textbf{ICEWS}} & \textit{\textbf{StaId}} \\
      \midrule
      PSL                    & \textbf{55.92} & \textbf{57.81} & \textbf{48.50} \\ 
      PSL$_{TF-IDF}$ w/o SI  & 52.07          & 56.70          & 46.45          \\
      PSL$_{BM25}$   w/o SI  & 51.87          & 57.22          & 45.94          \\
      PSL$_{Emb}$ w/o SI     & 52.96          & 57.16          & 46.69          \\
      PSL$_{LR}$     w/o SI  & 53.81          & 57.34          & 47.10          \\
      \bottomrule
      \end{tabular}
    }
    \caption{Performance of different variants of PSL. SI denotes the procedure of stance inference.}
    \label{p1}
  \end{minipage}
\end{figure*}
